Visibility Guided NMS: Efficient Boosting of Amodal Object Detection in Crowded Traffic Scenes

Object detection is an important task in environment perception for autonomous driving. Modern 2D object detection frameworks such as Yolo, SSD or Faster R-CNN predict multiple bounding boxes per object that are refined using Non-Maximum-Suppression (NMS) to suppress all but one bounding box. While object detection itself is fully end-to-end learnable and does not require any manual parameter selection, standard NMS is parametrized by an overlap threshold that has to be chosen by hand. In practice, this often leads to an inability of standard NMS strategies to distinguish different objects in crowded scenes in the presence of high mutual occlusion, e.g. for parked cars or crowds of pedestrians. Our novel Visibility Guided NMS (vg-NMS) leverages both pixel-based as well as amodal object detection paradigms and improves the detection performance especially for highly occluded objects with little computational overhead. We evaluate vg-NMS using KITTI, VIPER as well as the Synscapes dataset and show that it outperforms current state-of-the-art NMS.

==> result_table_amodal_allboxes.tex <==
% !TeX root = neurips_2019_ml4ad.tex

\begin{table}
  \caption{Averate Precision (AP) results of different NMS variants for amodal object detection. Evaluation was performed on the validation splits of each dataset. All GT boxes are used for evaluation including boxes with a size of smaller than $20 \times 20$\, px. Hybrid NMS outperforms both standard and Soft NMS and shows excellent performance in combination with Soft NMS.}
  \label{tab:map_results_amodal_allboxes}
  \centering
\begin{tabular}{ll|rrrr|rr}
\toprule
                       &       & \multicolumn{4}{c|}{AP [\%]} & & \\  
                       &                   & Car & Truck & Bus & Person & mAP [\%] & Runtime \\ \midrule
\multirow{4}{*}{KITTI \cite{geiger2012we}} & Standard NMS      &     &       &     &            &     &         \\ \cmidrule{2-8}
                       & Soft          &     &       &     &            &     &         \\ %best snapshot 296595
                       & Hybrid        &     &       &     &            &     &         \\
                       & Hybrid + Soft  &     &       &     &            &     &         \\
\midrule
\multirow{4}{*}{VIPER \cite{richter2017playing}} & Standard NMS      &     &       &     &            &     &         \\ \cmidrule{2-8}
                       & Soft           &     &       &     &            &     &         \\
                       & Hybrid         &     &       &     &            &     &         \\
                       & Hybrid + Soft  &     &       &     &            &     &         \\
\midrule
\multirow{4}{*}{Syncapes \cite{wrenninge2018synscapes}} & Standard NMS     & \num{60,74}&\num{56.47}&\num{56.39}&\num{69.94}&\num{60.88}&\textbf{\SI{29.1}{\milli\second}}\\ \cmidrule{2-8} %best snapshot 296595
                       & Soft           &     &       &     &            &     &         \\
                       & Hybrid          & \textbf{\num{64.01}}&\textbf{\num{56.86}}&\textbf{\num{56.23}}&\textbf{\num{71.51}}&\num{62.15}&\SI{29.3}{\milli\second}\\ %best snapshot 1285245
                       & Hybrid + Soft  &     &       &     &            &     &         \\
\bottomrule
\end{tabular}
\end{table}


